Hybrid Methods in Polynomial Optimisation

The Moment/Sum-of-squares hierarchy provides a way to compute the global minimizers of polynomial optimization problems (POP), at the cost of solving a sequence of increasingly large semidefinite programs (SDPs). We consider large-scale POPs, for which interior-point methods are no longer able to solve the resulting SDPs. We propose an algorithm that combines a first-order method for solving the SDP relaxation, and a second-order method on a non-convex problem obtained from the POP. The switch from the first to the second-order method is based on a quantitative criterion, whose satisfaction ensures that Newton's method converges quadratically from its first iteration. This criterion leverages the point-estimation theory of Smale and the active-set identification. We illustrate the methodology to obtain global minimizers of large-scale optimal power flow problems.

==> shared.tex <==


\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithm}
\usepackage{algpseudocodex}

\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

\newcommand{\creflastconjunction}{, and~}

\newsiamremark{remark}{Remark}
\crefname{remark}{Remark}{Remarks}
\newsiamremark{example}{Example}
\crefname{example}{Example}{Examples}
\newsiamthm{assumption}{Assumption}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{proposition}{Proposition}{Propositions}



\newcommand{\TheTitle}{Hybrid Methods in Polynomial Optimisation}
\newcommand{\TheAuthors}{J. Aspman, G. Bareilles, V. Kungurtsev, J. Mare\v{c}ek, M. Tak\'a\v{c}}

\headers{\TheTitle}{\TheAuthors}

\title{{\TheTitle}\thanks{Submitted to the editors \today. The authors are ordered alphabetically.}}

\author{
  Johannes Aspman\thanks{Faculty of Electrical Engineering, Czech Technical University of Prague, the Czech Republic (\email{firstname.lastname@fel.cvut.cz}).}
  \and Gilles Bareilles\footnotemark[2]
  \and Vyacheslav Kungurtsev\footnotemark[2]
  \and Jakub Mare\v{c}ek\footnotemark[2]
  \and Martin Tak\'a\v{c}\thanks{Mohamed bin Zayed University of Artificial Intelligence, Masdar City, Abu Dhabi, United Arab Emirates  (\email{takac.mt@gmail.com}).}
}



\usepackage{amsopn}



\usepackage{amsmath}						%
\usepackage{amssymb}						%
\usepackage{amsfonts}						%
\usepackage{array}


\usepackage{mathtools}						%


\usepackage[utf8]{inputenc}							%
\usepackage[T1]{fontenc}						%
\usepackage[normalem]{ulem}




\colorlet{MyBlue}{DodgerBlue!75!Black}
\colorlet{MyGreen}{DarkGreen!85!Black}
\colorlet{MyGray}{White!75!Black}

\definecolor{chartreuse}{HTML}{288800}
\definecolor{dark_gray}{HTML}{111111}
\definecolor{light_gray}{HTML}{555555}
\definecolor{tomato}{HTML}{FF6347}
\definecolor{snow}{HTML}{F1F1F1}
\definecolor{whiteee}{HTML}{EEEEEC}

\definecolor{c1}{RGB}{238,102,119}
\definecolor{c2}{RGB}{68, 119, 170}
\definecolor{c3}{RGB}{102, 204, 238}
\definecolor{c4}{RGB}{34, 136, 51}
\definecolor{c5}{RGB}{204, 187, 68}
\definecolor{c6}{RGB}{238, 102, 119}
\definecolor{c7}{RGB}{170, 51, 119}
\definecolor{c8}{RGB}{187, 187, 187}


\definecolor{vibrant1}{HTML}{EE7733} %
\definecolor{vibrant2}{HTML}{0077BB} %
\definecolor{vibrant3}{HTML}{33BBEE} %
\definecolor{vibrant4}{HTML}{EE3377} %
\definecolor{vibrant5}{HTML}{CC3311} %
\definecolor{vibrant6}{HTML}{009988} %
\definecolor{vibrant7}{HTML}{BBBBBB} %

\definecolor{bright1}{HTML}{4477AA} %
\definecolor{bright2}{HTML}{EE6677} %
\definecolor{bright3}{HTML}{228833} %
\definecolor{bright4}{HTML}{CCBB44} %
\definecolor{bright5}{HTML}{66CCEE} %
\definecolor{bright6}{HTML}{AA3377} %
\definecolor{bright7}{HTML}{BBBBBB} %

\definecolor{light_blue}{HTML}{77AADD}
\definecolor{orange}{HTML}{EE8866}
\definecolor{light_yellow}{HTML}{EEDD88}
\definecolor{pink}{HTML}{FFAABB}
\definecolor{light_cyan}{HTML}{99DDFF}
\definecolor{mint}{HTML}{44BB99}
\definecolor{pear}{HTML}{BBCC33}
\definecolor{olive}{HTML}{AAAA00}
\definecolor{pale_grey}{HTML}{DDDDDD}
\definecolor{black}{HTML}{000000}


\usepackage{tikz}
\usetikzlibrary{calc,patterns,arrows}
\usetikzlibrary{tikzmark,shapes}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{matrix}
\usetikzlibrary{perspective}
\usetikzlibrary{external}

\usepackage{pgfplots}
\usepgfplotslibrary{groupplots}

\usepackage{graphicx,epstopdf} %
\usepackage[export]{adjustbox}
\usepackage[caption=false]{subfig} %


\usepackage{multicol}
\usepackage{arydshln}
\usepackage{multirow}
\usepackage{wrapfig}

\newcommand{\includetikzfig}[2][1]{
  \resizebox{#1\textwidth}{!}{
    \input{figures/#2.tex}
  }
}

\newenvironment{customlegend}[1][]{%
    \begingroup
    \csname pgfplots@init@cleared@structures\endcsname
    \pgfplotsset{#1}%
}{%
    \csname pgfplots@createlegend\endcsname
    \endgroup
}%

\def\addlegendimage{\csname pgfplots@addlegendimage\endcsname}

\usepackage{acronym}              %
\usepackage{booktabs}						%
\usepackage{latexsym}						%
\usepackage{paralist}						%
\usepackage{xspace}							%
\usepackage{placeins}
\usepackage{enumitem}
\renewcommand{\labelenumi}{\roman{enumi})} %

\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}


\usepackage{hyperref}
\hypersetup{
final,
colorlinks=true,
linktocpage=true,
pdfstartview=FitH,
breaklinks=true,
pdfpagemode=UseNone,
pageanchor=true,
pdfpagemode=UseOutlines,
plainpages=false,
bookmarksnumbered,
bookmarksopen=false,
bookmarksopenlevel=1,
hypertexnames=true,
pdfhighlight=/O,
urlcolor=Maroon,linkcolor=MyBlue!60!black,citecolor=DarkGreen!70!black,	%
pdftitle={},
pdfauthor={},
pdfsubject={},
pdfkeywords={},
pdfcreator={pdfLaTeX},
pdfproducer={LaTeX with hyperref}
}

\usepackage{autonum}






\usepackage{color-edits}
\addauthor{gb}{DodgerBlue}
\addauthor{JM}{orange}
\addauthor{JA}{red}


\newcommand{\old}[1]{{\color{gray}#1}}		%
\newcommand{\needref}[1]{{\color{red} [!!]}}		%


\newcommand{\ie}{\emph{i.e.},\xspace}
\newcommand{\eg}{\emph{e.g.},\xspace}

\newcommand{\debug}[1]{#1}                                  %

\newcommand{\newmacro}[2]{\newcommand{#1}{\debug{#2}}}		%
\newcommand{\newalgo}[2]{\newcommand{#1}{\debug{\textsc{#2}}\xspace}}		%
\newcommand{\newop}[2]{\DeclareMathOperator{#1}{\debug{#2}}}		%




\newmacro{\ab}{$\alpha$-$\beta$}

\newmacro{\R}{\mathbb{R}}
\newmacro{\N}{\mathbb{N}}
\newmacro{\RR}{\mathbb{R}}
\newmacro{\bbR}{\mathbb{R}}
\newmacro{\bbN}{\mathbb{N}}

\newmacro{\E}{\mathcal{E}}
\newmacro{\I}{\mathcal{I}}
\newmacro{\mE}{m_\mathcal{E}}
\newmacro{\mI}{m_\mathcal{I}}


\newmacro{\C}{\mathbb{C}}

\newmacro{\xtilde}{\tilde x}
\newmacro{\x}{x}
\newmacro{\y}{y}
\newmacro{\stepsize}{\eta}
\newmacro{\st}{\text{s.t.}}

\newmacro{\mfR}{\Re}
\newmacro{\mfI}{\Im}
\newmacro{\RK}{R^{(k)}}


\newop{\trace}{trace}
\newop{\tr}{tr}
\newop{\dist}{dist}

\newmacro{\eqdef}{\triangleq}

\newmacro{\nhd}{\mathcal{N}}
\newmacro{\ball}{\mathcal{B}}


\newcommand\tagthis{\addtocounter{equation}{1}\tag{\theequation}}

\newcommand{\vx}{\debug{x}}                  %
\newcommand{\vPsys}{\debug{z}}               %
\newcommand{\opt}[1][\vx]{{#1}^{\debug{\star}}}  %
\newcommand{\crit}[1][\vx]{\debug{\bar{#1}}} %
\newcommand{\adh}[1][\vx]{\debug{\hat{#1}}}  %

\newcommand{\curr}[1][\vx]{{#1}^{\debug{k}}}  %
\newcommand{\prev}[1][\vx]{{#1}^{\debug{k-1}}}%
\newcommand{\nextit}[1][\vx]{{#1}^{\debug{k+1}}}  %

\newmacro{\Lag}{\mathcal{L}}  %
\newcommand{\redLag}[1]{\Lag^{#1}}  %

\newcommand{\Sym}[1]{\mathcal{\debug{S}}_{#1}}
\newcommand{\SymPD}[1]{\mathcal{\debug{S}}_{#1}^+}

\newmacro{\idfun}{r}
\newmacro{\Actset}{\mathcal{A}}
\newmacro{\Psys}{F}
\newmacro{\Psysn}{p}
\newmacro{\Psysm}{q}

\newmacro{\Sol}{\mathcal{S}}
\newmacro{\SolDual}{\Sol_{\mathcal{D}}}

\newmacro{\dualSet}{\bbR^{\mE}\times\bbR^{\mI}_{+}}

\newmacro{\bigoh}{\mathcal{O}}


\newmacro{\D}{\operatorname{D}}     %
\newmacro{\Jac}{\operatorname{Jac}} %
\newmacro{\diag}{\operatorname{diag}}
\newmacro{\rank}{\operatorname{rank}}

\newmacro{\degree}{\operatorname{deg}}
\newmacro{\parts}{\mathcal{P}}





\usepackage[textsize=tiny]{todonotes}
\newcommand{\mt}[1]{\todo[color=pink,inline]{#1}}
\newcommand{\gb}[1]{\todo[color=DodgerBlue,inline]{#1}}

